Learning Nonlinear Couplings in Network of Agents from a Single Sample Trajectory

We consider a class of stochastic dynamical networks whose governing dynamics can be modeled using a coupling function. It is shown that the dynamics of such networks can generate geometrically ergodic trajectories under some reasonable assumptions. We show that a general class of coupling functions can be learned using only one sample trajectory from the network. This is practically plausible as in numerous applications it is desired to run an experiment only once but for a longer period of time, rather than repeating the same experiment multiple times from different initial conditions. Building upon ideas from the concentration inequalities for geometrically ergodic Markov chains, we formulate several results about the convergence of the empirical estimator to the true coupling function. Our theoretical findings are supported by extensive simulation results.

==> [TCNS]-Learning Couplings for multi-agent system from single trajectory/Files/Mydef.tex <==

\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsbsy}
\usepackage{latexsym}
\usepackage{amsmath} % assumes amsmath package installed
% \usepackage{amssymb,latexsym,amsmath,amsthm}
% \usepackage{xcolor}
\usepackage{epsfig,psfrag,color}
%\usepackage[ruled]{algorithm2e}
\usepackage[ruled,linesnumbered]{algorithm2e}
\SetKwRepeat{Do}{do}{while}%
%\usepackage[notref,notcite]{showkeys}
\usepackage{graphicx}
%\usepackage{epsfig,psfrag}

\usepackage[noend]{algpseudocode}
\usepackage{booktabs}
\usepackage{siunitx}% An awesome package for typesetting and manipulation numbers and units.
\usepackage{hyperref}% Used for insert the link
\usepackage{courier}% courier font
\usepackage{comment}


\usepackage{caption}% Better control over caption
% \captionsetup{font=small}
\usepackage{lipsum}% Example text
\usepackage{multirow}
\usepackage{diagbox} 
%\usepackage{subfig}
\usepackage{subcaption}
% \usepackage{mnsymbol}
%% Added Packages===============================Guangyi
% \usepackage{booktabs}% for tables
% \usepackage{caption}% Better control over caption
% \captionsetup{font=small}
% \usepackage{subcaption}
\usepackage{biblatex}
\addbibresource{Ref.bib}
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}


\newcommand{\SP}{\hspace{2pt}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\tE}{\mathcal{E}}
% \newcommand{\tx}{\Tilde{x}}
%\newcommand{\x}{{\bf x}}
\newcommand{\x}{x}
\newcommand{\m}{{ m}}
\newcommand{\br}{{\rm r}}
%\newcommand{\X}{{\bf X}}
\newcommand{\X}{x}
\newcommand{\Xc}{\mathcal{X}}
%\newcommand{\W}{{\bf W}}
\newcommand{\W}{{w}}
\newcommand{\V}{{\bf V}}
% \newcommand{\bu}{{\bf u}}
%\newcommand{\w}{{\bf w}}
\newcommand{\w}{w}
% \newcommand{\bc}{{\bf c}}
% \newcommand{\bR}{{\bf R}}
\newcommand{\bP}{{\bf  P}}
\newcommand{\Prb}{\mathbb{P}}
% \newcommand{\ty}{\Tilde{y}}
\newcommand{\I}{\bf {I}}

\newcommand{\Ni}{\mathcal{N}_i}
\newcommand{\A}{{\bf A}}
\newcommand{\B}{{\bf B}}
\newcommand{\C}{{\bf C}}
\newcommand{\F}{{ F}}
\newcommand{\G}{{\bf G}}
\newcommand{\Hf}{\mathcal{H}}
\newcommand{\NI}{\mathcal{N}_i}
\newcommand{\Cm}{\mathcal{C}}
\newcommand{\Sigm}{\sigma_\mathcal{M}}
\newcommand{\Dj}{\mathcal{D}_j}
\newcommand{\Cov}{\text{Cov}}
\newcommand{\Var}{\text{Var}}
\newcommand{\Ltw}{{L^{2, *}_{{\rho_T}}}}
\newcommand{\bgp}{\bar g_\psi}

\definecolor{amber}{rgb}{1.0, 0.49, 0.0}
\newcommand{\CR}{\color{red}}% Note
\newcommand{\CB}{\color{blue}}% Check
\newcommand{\CO}{\color{amber}}% Needs rewrite
\newcommand{\CG}{\color{green}}% take a look


\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\inner}[1]{\left\langle#1\right\rangle}
\newcommand{\normd}[1]{{\bf d}_{\mathcal{L}}\left[#1\right]}
\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1\langle}\)}%
  \mathopen{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1\rangle}\)}%
  \mathclose{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\makeatother





\DeclareMathOperator*{\minimize}{minimize}
\newcommand\vertarrowbox[3][2ex]{%
	\begin{array}[t]{@{}c@{}} #2 \\
		\left\uparrow\vcenter{\hrule height #1}\right.\kern-\nulldelimiterspace\\
		\makebox[0pt]{\scriptsize#3}
	\end{array}%
}


\newtheorem{thm}{\bf Theorem}
\newtheorem{rem}{\bf Remark}
\newtheorem{lem}{\bf Lemma}
\newtheorem{Prop}{\bf Proposition}
\newtheorem{defn}{\bf Definition}
\newtheorem{cor}{\bf Corollary}
\newtheorem{asm}{\bf Assumption}
\newtheorem{exmp}{\bf Example}








\bgroup
\def\arraystretch{1.3}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

